KD3A: Unsupervised Multi-Source Decentralized Domain Adaptation via Knowledge Distillation

Conventional unsupervised multi-source domain adaptation (UMDA) methods assume all source domains can be accessed directly. This neglects the privacy-preserving policy, that is, all the data and computations must be kept decentralized. There exists three problems in this scenario: (1) Minimizing the domain distance requires the pairwise calculation of the data from source and target domains, which is not accessible. (2) The communication cost and privacy security limit the application of UMDA methods (e.g., the domain adversarial training). (3) Since users have no authority to check the data quality, the irrelevant or malicious source domains are more likely to appear, which causes negative transfer. In this study, we propose a privacy-preserving UMDA paradigm named Knowledge Distillation based Decentralized Domain Adaptation (KD3A), which performs domain adaptation through the knowledge distillation on models from different source domains. KD3A solves the above problems with three components: (1) A multi-source knowledge distillation method named Knowledge Vote to learn high-quality domain consensus knowledge. (2) A dynamic weighting strategy named Consensus Focus to identify both the malicious and irrelevant domains. (3) A decentralized optimization strategy for domain distance named BatchNorm MMD. The extensive experiments on DomainNet demonstrate that KD3A is robust to the negative transfer and brings a 100x reduction of communication cost compared with other decentralized UMDA methods. Moreover, our KD3A significantly outperforms state-of-the-art UMDA approaches.

==> content/ethic_statement.tex <==
\section{Ethics statement}
We address a decentralized domain adaptation paradigm to solve the domain shift problem under the privacy-preserving policy. We offer the possible influence of our work from three aspects: fundamental theory impact, machine learning application impact, and social impact.

For the fundamental theory impact, we analyze the knowledge distillation in domain adaptation from a theoretical perspective and derive a new generalization bound for it. The new theoretical bound will inspire further studies of the following two challenges: how to theoretically describe the knowledge quality and how to bridge the domain gap without accessing data.

For the machine learning application impact, we evaluate our paradigm under the large-scale real-world datasets and show it can be applied to non-laboratory environments such as data markets.

For the social impact, our work owns two properties: decentralization and privacy protection. Therefore, it is friendly to the data providers and the governments that pay attention to the privacy-preserving policy, e.g., the general data protection regulation in the European Union.


